Examining Pathological Bias in a Generative Adversarial Network Discriminator: A Case Study on a StyleGAN3 Model

Generative adversarial networks (GANs) generate photorealistic faces that are often indistinguishable by humans from real faces. While biases in machine learning models are often assumed to be due to biases in training data, we find pathological internal color and luminance biases in the discriminator of a pre-trained StyleGAN3-r model that are not explicable by the training data. We also find that the discriminator systematically stratifies scores by both image- and face-level qualities and that this disproportionately affects images across gender, race, and other categories. We examine axes common in research on stereotyping in social psychology.

==> sections/methods.tex <==
\section{Experiments and Results}


In Study 1, we examine how the discriminator evaluates faces from the FFHQ dataset--the face image dataset it was trained on. In Study 2, we examine how the discriminator evaluates a novel set of faces scraped from Google. 

\subsection{Correlation with Image Luminance}

As a motivating experiment, we examine the relationship of luminance to the score assigned by the GAN.  In the GAN, images are encoded in an red-green-blue (RGB) color channel representation; from these, we can extrapolate a luminance value. The (photometric) \textbf{luminance} score~\cite{stone2016field} is a measure of light intensity for a particular area, the objective counterpart to subjective \textit{brightness}.  Relative luminance $Y \in [0,1]$ normalized luminance such that $1.0$ is reference white and $0.0$ is the darkest black.  Relative luminance can be calculated from the RGB channel representation of an image with Equation~\ref{eq:luminance} where $R$, $G$, and $B$ are the respective values for red, green, and blue, normalized to $[0,1]$~\cite{sugawara2014ultra}.
\begin{equation}
Y = (0.2126)R + (0.7152)G + (0.0722)B
\label{eq:luminance}
\end{equation}

We calculate the relative luminance intensity of every image in the FFHQ dataset and cross-reference this with the score assigned to the image by the discriminator. Figure~\ref{fig:luminance_correlation} shows a clear linear relationship between the luminance value and the score assigned to the image by the discriminator~(Figure~\ref{fig:luminance_correlation}). The 95\% highest-density region (HDR)\footnote{A 95\% HDR or HDI indicates that 95\% of the data or distribution falls within the range shown.}

\begin{figure}[t!]
\centering
\includegraphics[scale=0.4]{figures/luminance_hdr.pdf}
\caption{Discriminator score as a function of luminance with a superimposed linear regression in the FFHQ dataset.  Colors show HDRs from 50\%-95\%.  The discriminator shows a clear preference for face photos with higher luminance. The scores increase roughly linearly with luminance.  But the 95\% shows that this is not because high luminance images are especially common. This can be seen even more clearly in Figure~\ref{fig:luminance_dist}.}

\label{fig:luminance_correlation}
\end{figure}
\begin{figure}[t!]
\centering
\includegraphics[scale=0.4]{figures/luminance_dist.pdf}
\caption{Distribution of luminance over the training dataset.  The 95\% HDI shows that that vast majority of the data do not have especially high luminance, so this cannot explain the model's preference for it.}

\label{fig:luminance_dist}
\end{figure}


\subsection{Discriminator Bias for Lighter Skin Tones}

\begin{comment}
    
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/atypical_mens_face_race_dist_aggregate.pdf}
    %\includesvg[width=\linewidth, height=6cm]{figures/atypical_mens_face_dist.svg}
    \caption{
 Caption here.
    }
    \label{fig:race_distribution}
\end{figure}
\end{comment}


\subsection{Labeled Faces Data Collection}

While the correlation of score with luminance is compelling, we wish to know the degree to which the GAN's discriminator penalizes faces based on race.  
To examine this, we via Google image search to find faces of men and women of each of three perceived races: Asian, Black, and white. We recruited participants from Prolific (an online crowdsourcing platform) to label both these images, as well as the top and bottom 100 images from Study 1, for perceived race with choices determined by US Census categories. Of interest for our purposes here are the categories \textit{Black or African American}, \textit{Asian or Pacific Islander}, and \textit{White}.  We  ask participants for categorical labels for race.  We also elicit ratings for skin tone, hair length, Asiocentricity, Afrocentricity, and Eurocentricity, with a 1-7 scale for each. We use the crowdsourced categorical labels for race to verify the authenticity of the labels and remove from the dataset those for which there is less than 2/3 agreement among raters.  We then manually inspect for obviously mislabeled images, which we remove. From those that remain, for each gender, we take 100 images for each race (50 with long hair, and 50 with short).  We thus have $100\times 3 = 300$ images per gender.

For the initial search, We use the following search terms, substituting the appropriate gender and race: \texttt{[race] [gender] with long hair, Black men with locs\footnote{We use this for Black men because ``Black men with short hair'' returned ambiguous and inconsistent results due to differing perceptions about what constitutes ``short hair'' for Black men.}, [race] [gender] with buzz cut}.  These search terms were chosen so that we would have a variety of faces with different hair styles. Since prior research has shown that the ``average face'' in the FFHQ dataset is a white woman~\cite{salminen2020analyzing}, we hypothesized that more gender-atypical hair styles would attenuate the results.  Images were cropped so that they only contained the face.


A fair discriminator would not show substantial differences between each group.  However, this is not what we find. Figure~\ref{fig:race_distribution} shows clear differences between the discriminator-assigned scores for each race and hair style.  For men, long hair consistently penalizes the score: the effect is least pronounced for Asian men, but both black and white men see huge penalties, with long-haired black men's scores being the lowest and most entropic any group.
The faces of white men with short hair are heavily skewed toward the high end with a long tail on the low end.  Being non-white or having long hair both increase the entropy of the distribution for men.

The situation is quite different for women.  Asian and white women show no substantial difference in score based on hair type.  Black women, however, are penalized for having long hair.  Women's assigned score distributions all have long tails on the left, which is not the case for men. It is surprising that the mode of white men's faces is so much higher and shifted to the right than that of women's faces, given that the ``average face'' of the training data is a white women.

 
\begin{figure*}[t!]

\centering
\includegraphics[width=0.95\linewidth]{figures/atypical_all_50face_dist.pdf}
\caption{Density plots for the faces labeled men (left) and women (right) for each race. White men with short hair were scored substantially higher than those of any other group, though those with long hair are penalized heavily. Black men with long hair have the highest entropy distribution.  The differences in score for women's faces are mostly nonexistent, with the exception of black women, who are favored with short hair.  Asian faces do not show much difference between any group. Note the consistent long left tails on the distributions of women versus men.}

\label{fig:hair_dists}

    
\end{figure*}
\begin{comment}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/atypical_mens_face_dist.pdf}
         \caption{Scores of faces labeled men}
         \label{fig:men_hair_dist}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/atypical_womens_face_dist.pdf}
         \caption{Scores of Faces labeled women}
         \label{fig:women_hair_dist}
     \end{subfigure}
\label{fig:hair_dists}
\caption{Consistently, across faces labeled as both men and women, shorter hair was preferred, though the effect is much more pronounced for faces labeled as men.  Black men's faces have the highest entropy distributions, by far.  Black women's faces, interestingly, do not show a similar trend, and the scores assigned to  women's faces in general are not as stratified by race.\alvin{Note to self: fix capitalization of race names}}
\end{figure*}
\end{comment}




\subsection{Stark Differences at the Tails}
\begin{figure*}[t!]
\centering
\begin{minipage}[t]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/top100.png}
   % \caption{100 highest-scoring faces}
   % \label{fig:top100}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.5\linewidth}
    \includegraphics[width=\textwidth]{figures/least100.png}
    %\caption{100 lowest-scoring faces}
    %\label{fig:least100}
\end{minipage} 

\caption{100 highest-scoring and lowest-scoring faces according to StyleGAN 3's discriminator. While occasional examples of faces with lighter skin receive a low score in a dark image, the stark bias for lighter-skinned faces and against darker-skinned ones is clear.  There is a propensity to favor the color pink.  There is not one apparent Black person's face in the top 100.
}
\label{fig:topbottom100}
\end{figure*}
\ryan{i feel like Fig. 4 should become Fig 3, since it's about the FFHQ faces and not the Google ones}
But how does this look in practice?  To get an impression of the implication of this bias on a large dataset, we score every image in the FFHQ dataset and sort by discriminator score, examining the top-scoring and lowest-scoring 100 images.  The results, shown in Figure~\ref{fig:topbottom100}, are striking.  The StyleGAN 3 model shows a remarkable bias for lighter faces and brighter images, with some apparent color bias, as well, with pink hair appearing in many of the top-scoring images.  Since pink hair is uncommon in the dataset, the color bias cannot be explained by similar colors' frequency in the training data.  It may be due to a learned association with lighter skin tones.  In short, darker faces are more likely to be classified as fake by the discriminator. 

\alvin{There's related work on CNNs/facial recognition software that would be relevant here.}

\begin{comment}
\begin{figure}[]
%PDF is too slow to load.
    \centering
    \includegraphics[scale=0.5]{figures/training_color_scatter.png}
    %\includesvg[width=\linewidth, height=6cm]{figures/atypical_mens_face_dist.svg}
    \caption{
 Caption here.
    }
    \label{fig:race_distribution}
\end{figure}

\begin{figure}[]
    %centering
    \includegraphics[scale=0.5]{figures/training_color_histogram_logscale.pdf}
    \caption{Log Scale}
    \label{fig:color_histogram}
\end{figure}
\end{comment}
\begin{figure*}[t]
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/training_color_scatter.png}
         \caption{This is the same correlation shown in Figure~\ref{fig:luminance_correlation}, but with each of the 60,000 squares displaying the mean color of the image.  As shown in Figure~\ref{fig:luminance_correlation}, score increases with luminance, but along the $y$-axis, darker tones are generally scored lower at any given $x$ coordinate.  Cooler  hues are penalized, and red is rewarded, with several red outliers.  We see visually that the variance in score correlated with the variance in color.} 
         \label{fig:mean_color_scatter}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/training_color_histogram_logscale.pdf}
         \caption{Histogram of 60,000 training photos binned by the mean discriminator score. The color of each bar is the mean color of the images within the given score range. The smooth transition from darker to lighter skin colors (and finally to red and pink) is remarkable.  Darker skin tones are dispreferred, but red is peculiarly rewarded. The right extremum, though an extremely small part of the training data and not a typical skin color, has exceptionally  high average scores. This appears pathological.}
         \label{fig:color_histogram}
        
     \end{subfigure}
     \caption{The color composition of the images is highly correlated with the score, beyond that which can be accounted for by luminance alone.  Though luminance is correlated with higher score, so is larger amounts of the color red.  We cannot account for this due to the composition of the training data, since this \textit{is} the training data, and  many of the highest scoring faces occur \textit{less} frequently.}
     \label{fig:color_charts}
\end{figure*}










